Emergent Outcomes of the veToken Model

Decentralised organisations use blockchains for governance: on-chain transactions allocate voting weight, publish proposals, cast votes, and enact the results. A key challenge is aligning the short-term outlook of pseudonymous voters with the long-term success of the organisation. The Vote-Escrowed Token (veToken) model attempts to resolve this tension by requiring voters to lock tokens of value for an extended period in exchange for voting weight. In this paper we describe the veToken model and analyse its emergent outcomes. We describe its implementation by Curve, a popular automated market maker for stablecoins, and the ecosystem of protocols built on top. We show that voting outcomes are strongly associated with the bribes set by higher-level protocols, and that the cost per vote varies depending on how it is acquired. The outcomes of the fortnightly votes held by Convex Finance closely track the distribution of bribes through voting markets such as Votium. Frax Finance, a stablecoin issuer, plays a central role even though it directly locks relatively few tokens with Curve; instead, it indirectly locks tokens through yield aggregators and purchases voting weight through voting markets. Although the veToken model in isolation is straightforward, it leads to complex and emergent outcomes. Decentralised organisations should consider these outcomes before adopting the model.

==> acronyms.tex <==
\newacronym{api}{API}{application programming interface}
\newacronym{dao}{DAO}{Decentralised Autonomous Organisation}
\newacronym{ens}{ENS}{Ethereum Name Service}
\newacronym{nft}{NFT}{non-fungible token}
\newacronym{roi}{RoI}{Republic of Ireland}
\newacronym{setu}{SETU}{South East Technological University}

